Scaling Pareto-Efficient Decision Making Via Offline Multi-Objective RL

The goal of multi-objective reinforcement learning (MORL) is to learn policies that simultaneously optimize multiple competing objectives. In practice, an agent's preferences over the objectives may not be known apriori, and hence, we require policies that can generalize to arbitrary preferences at test time. In this work, we propose a new data-driven setup for offline MORL, where we wish to learn a preference-agnostic policy agent using only a finite dataset of offline demonstrations of other agents and their preferences. The key contributions of this work are two-fold. First, we introduce D4MORL, (D)atasets for MORL that are specifically designed for offline settings. It contains 1.8 million annotated demonstrations obtained by rolling out reference policies that optimize for randomly sampled preferences on 6 MuJoCo environments with 2-3 objectives each. Second, we propose Pareto-Efficient Decision Agents (PEDA), a family of offline MORL algorithms that builds and extends Decision Transformers via a novel preference-and-return-conditioned policy. Empirically, we show that PEDA closely approximates the behavioral policy on the D4MORL benchmark and provides an excellent approximation of the Pareto-front with appropriate conditioning, as measured by the hypervolume and sparsity metrics.

==> tables/main_exp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\small
\begin{tabular}{lllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{2}{*}{Metric}} & \multicolumn{1}{c}{\multirow{2}{*}{MODT-P}} & \multicolumn{1}{c}{\multirow{2}{*}{RvS-P}} & \multicolumn{1}{c}{\multirow{2}{*}{BC-P}} & \multicolumn{1}{c}{\multirow{2}{*}{MODT-N}} & \multicolumn{1}{c}{\multirow{2}{*}{RvS-N}} & \multicolumn{1}{c}{\multirow{2}{*}{BC-N}} \\
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                         & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                      & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                      \\ \hline
\multirow{6}{*}{Ant}                       & \multirow{2}{*}{Exp}                         & HV(e6)                                      & 6.02$\pm$.02                                & 6.24$\pm$.07                               & 4.49$\pm$.3                               & 5.10$\pm$.16                                & 5.05$\pm$.07                               & 0.78$\pm$.57                              \\  
                                           &                                              & SP(e4)                                      & 7.06$\pm$1.29                               & 4.55$\pm$.59                               & 32.1$\pm$12.2                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{nExp}                        & HV                                          & 5.99$\pm$.01                                & 4.37$\pm$1.88                              & 4.42$\pm$.62                              & 4.71$\pm$.33                                & 3.49$\pm$.05                               & 2.42$\pm$.17                              \\  
                                           &                                              & SP                                          & 5.46$\pm$.44                                & 5.21$\pm$.34                               & 17.3$\pm$8.03                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{Med}                         & HV                                          & 5.60$\pm$.03                                & 5.94$\pm$.04                               & 4.35$\pm$.07                              & 3.34$\pm$.71                                & 4.91$\pm$.06                               & 2.34$\pm$.09                              \\  
                                           &                                              & SP                                          & 6.56$\pm$.45                                & 4.96$\pm$ 1.1                              & 11.7$\pm$6.45                             &                                             &                                            &                                           \\ \hline
\multirow{6}{*}{Cheetah}                   & \multirow{2}{*}{Exp}                         & HV(e6)                                      & 5.69$\pm$.01                                & 5.77$\pm$.004                              & 5.52$\pm$.04                              & 5.59$\pm$.05                                & 4.56$\pm$.56                               & 1.45$\pm$.04                              \\  
                                           &                                              & SP(e4)                                      & 1.44$\pm$.28                                & 0.74$\pm$.03                               & 1.69$\pm$.70                              &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{nExp}                        & HV                                          & 5.71$\pm$.006                               & 5.77$\pm$.01                               & 5.58$\pm$.04                              & 5.38$\pm$.14                                & 3.88$\pm$.15                               & 1.57$\pm$.08                              \\  
                                           &                                              & SP                                          & 1.02$\pm$.16                                & 0.67$\pm$.04                               & 1.05$\pm$.29                              &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{Med}                         & HV                                          & 5.64$\pm$.006                               & 5.77$\pm$.002                              & 5.26$\pm$.06                              & 5.51$\pm$.01                                & 5.28$\pm$.35                               & 3.14$\pm$.38                              \\  
                                           &                                              & SP                                          & 0.81$\pm$.52                                & 0.31$\pm$.005                              & 2.18$\pm$.49                              &                                             &                                            &                                           \\ \hline
\multirow{6}{*}{Hopper-v2}                 & \multirow{2}{*}{Exp}                         & HV(e7)                                      & 1.92$\pm$.01                                & 1.98$\pm$.02                               & 1.40$\pm$.03                              & 1.60$\pm$.04                                & 1.72$\pm$.04                               & 0.82$\pm$.42                              \\  
                                           &                                              & SP(e5)                                      & 8.89$\pm$1.84                               & 1.91$\pm$.51                               & 23.7$\pm$20.1                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{nExp}                        & HV                                          & 1.77$\pm$.12                                & 1.42$\pm$.61                               & 1.39$\pm$.05                              & 1.47$\pm$.03                                & 1.60$\pm$.02                               & 0.71$\pm$.41                              \\  
                                           &                                              & SP                                          & 6.70$\pm$.98                                & 1.44$\pm$.14                               & 25.9$\pm$20.8                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{Med}                         & HV                                          & 1.82$\pm$.02                                & 1.80$\pm$.27                               & 1.56$\pm$.01                              & 1.54$\pm$.08                                & 1.42$\pm$.04                               & 0.48$\pm$.48                              \\  
                                           &                                              & SP                                          & 1.54$\pm$.69                                & 1.75$\pm$.52                               & 9.57$\pm$8.64                             &                                             &                                            &                                           \\ \hline
\multirow{6}{*}{Hopper-v3}                 & \multirow{2}{*}{Exp}                         & HV(e10)                                     & 3.24$\pm$.09                                & 3.27$\pm$.1                                & 2.29$\pm$.29                              & 1.22$\pm$.27                                & 2.33$\pm$.14                               & 0.03$\pm$.007                             \\  
                                           &                                              & SP(e5)                                      & 1.42$\pm$.42                                & 1.11$\pm$.22                               & 0.75$\pm$.145                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{nExp}                        & HV                                          & 3.37$\pm$.01                                & 3.16$\pm$.03                               & 2.57$\pm$.11                              & 1.62$\pm$.03                                & 1.76$\pm$.24                               & 0.02$\pm$.003                             \\  
                                           &                                              & SP                                          & 0.86$\pm$.02                                & 0.89$\pm$.16                               & .617$\pm$.07                              &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{Med}                         & HV                                          & 2.63$\pm$.17                                & 2.98$\pm$.06                               & 2.31$\pm$.16                              & 1.72$\pm$.12                                & 1.57$\pm$.08                               & 0.13$\pm$.04                              \\  
                                           &                                              & SP                                          & 4.59$\pm$1.51                               & 1.04$\pm$.28                               & 0.79$\pm$.191                             &                                             &                                            &                                           \\ \hline
\multirow{6}{*}{Swimmer}                   & \multirow{2}{*}{Exp}                         & HV(e4)                                      & 3.16$\pm$.005                               & 3.22$\pm$.007                              & 3.21$\pm$.008                             & 2.49$\pm$.28                                & 3.19$\pm$.007                              & 1.81$\pm$.03                              \\  
                                           &                                              & SP(e0)                                      & 12.1$\pm$6.49                               & 5.00$\pm$.42                               & 3.79$\pm$1.03                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{nExp}                        & HV                                          & 3.11$\pm$.01                                & 3.23$\pm$.005                              & 3.22$\pm$.008                             & 2.59$\pm$.09                                & 3.23$\pm$.003                              & 1.98$\pm$.14                              \\  
                                           &                                              & SP                                          & 5.95$\pm$1.14                               & 3.42$\pm$.22                               & 3.82$\pm$.64                              &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{Med}                         & HV                                          & 2.83$\pm$.04                                & 2.76$\pm$.02                               & 2.81$\pm$.04                              & 6.72$\pm$1.04                               & 2.78$\pm$.01                               & 0.46$\pm$.14                              \\  
                                           &                                              & SP                                          & 2.74$\pm$1.51                               & 1.53$\pm$.1                                & 1.21$\pm$.07                              &                                             &                                            &                                           \\ \hline
\multirow{6}{*}{Walker2d}                  & \multirow{2}{*}{Exp}                         & HV(e6)                                      & 4.84$\pm$.1                                 & 5.15$\pm$.009                              & 3.47$\pm$.13                              & 0.61$\pm$.43                                & 4.95$\pm$.06                               & 0.07$\pm$.009                             \\  
                                           &                                              & SP(e4)                                      & 5.28$\pm$.99                                & 1.91$\pm$.25                               & 46.9$\pm$23.2                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{nExp}                        & HV                                          & 5.05$\pm$.01                                & 5.15$\pm$.18                               & 2.90$\pm$.47                              & 0.57$\pm$.23                                & 4.97$\pm$.04                               & 0.06$\pm$.003                             \\  
                                           &                                              & SP                                          & 4.18$\pm$.76                                & 1.99$\pm$.33                               & 68.3$\pm$33.6                             &                                             &                                            &                                           \\ \cline{2-9} 
                                           & \multirow{2}{*}{Med}                         & HV                                          & 3.17$\pm$.14                                & 4.96$\pm$.02                               & 2.93$\pm$.75                              & 2.62$\pm$.81                                & 4.21$\pm$2.74                              & 1.19$\pm$.21                              \\  
                                           &                                              & SP                                          & 30.7$\pm$13.6                               & 2.10$\pm$.17                               & 154$\pm$144                               &                                             &                                            &                                           \\  \hline
\end{tabular}
\label{main_exp_table}
\caption{\textbf{Full experiment results for \texttt{uniform} datasets}}
\end{table}
